Spectrum of conformal gauge theories on a torus

Many model quantum spin systems have been proposed to realize critical points or phases described by 2+1 dimensional conformal gauge theories. On a torus of size $L$ and modular parameter $\tau$, the energy levels of such gauge theories equal $(1/L)$ times universal functions of $\tau$. We compute the universal spectrum of QED$_3$, a U(1) gauge theory with $N_f$ two-component massless Dirac fermions, in the large $N_f$ limit. We also allow for a Chern-Simons term at level $k$, and show how the topological $k$-fold ground state degeneracy in the absence of fermions transforms into the universal spectrum in the presence of fermions; these computations are performed at fixed $N_f/k$ in the large $N_f$ limit.

==> headersDraft.tex <==
\usepackage[margin=0.7in]{geometry}
%\usepackage[square,numbers]{natbib}
\usepackage{natbib}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{verbatim}
\usepackage{braket}
\usepackage{enumitem}
\DeclareGraphicsRule{*}{mps}{*}{}
\usepackage{feynmp}
\unitlength = 1mm
\usepackage{math tools} %\Aboxed{ } draws boxes around '&' in align
\usepackage{dsfont} %gives the ``double stroke 1" I like to use for the identity \mathds{}
\usepackage{mathrsfs} %give very curly math script. I use it for \hilb=\mathscr{H}, Hilbert space H 
%\usepackage{pbox} %for adding boxes not in equations
%\usepackage{undertilde} %for a tilde under a letter/symbol, such as in a simapprox
\usepackage{parskip} %removes automatic indenting of paragraphs
\usepackage{mathabx} %has sun symbol \Sun, (also: \Earth, \Moon)
\usepackage{multirow}
\usepackage{arydshln} %\hdashline
\usepackage{lscape}%\begin{landscape} -- \end{landscape} makes landscape pages
\usepackage{slashed}%gives Dirac slash -- \slashed(\partial) -- I make a shortcut below
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor} %coloured text

% allows line spacing changes
\usepackage{setspace}
\setstretch{1.06} % changes spacing

% From Subir's manuscript (doubles removed)
\usepackage{amssymb,mathrsfs,bm,xspace,soul} 
\usepackage{graphicx}  
\usepackage{color} 

\usepackage[colorlinks=true]{hyperref} 
\hypersetup{
    bookmarks=true,         % show bookmarks bar?
    unicode=false,          % non-Latin characters 
    pdftoolbar=true,        % show Acrobat
    pdfmenubar=true,        % show Acrobat 
    pdffitwindow=false,     % window fit to page when opened
    pdfstartview={FitH},    % fits the width of the page to the window
    pdftitle={My title},    % title
    pdfauthor={Author},     % author
    pdfsubject={Subject},   % subject of the document
    pdfcreator={Creator},   % creator of the document
    pdfproducer={Producer}, % producer of the document
    pdfkeywords={keyword1} {key2} {key3}, % list of keywords
    pdfnewwindow=true,      % links in new window
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=magenta, %red,          % color of internal links (change box color with linkbordercolor)
    citecolor=blue,        % color of links to bibliography
    filecolor=magenta,      % color of file links
    urlcolor=cyan           % color of external links
} 

%\usepackage{chngcntr} %counter
%\counterwithin{figure}{section}

% Special math character shortcuts


%\mathcal shortcuts
\newcommand{\ord}{\mathcal{O}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\hamk}{\mathcal{H}}
\newcommand{\bcX}{\boldsymbol{\mathcal{X}}}
\newcommand{\bcW}{\boldsymbol{\mathcal{W}}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\V}{\mathcal{V}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\D}{\mathcal{D}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\E}{\mathcal{E}}

%\mathscr shortcuts
\newcommand{\hilb}{\mathscr{H}}

%\mathbf shortcuts
\newcommand{\vn}{{\mathbf{n}}}
\newcommand{\vk}{{\mathbf{k}}}
\newcommand{\vr}{{\mathbf{r}}}
\newcommand{\vQ}{{\mathbf{Q}}}
\newcommand{\vK}{{\mathbf{K}}}
\newcommand{\vq}{{\mathbf{q}}}
\newcommand{\vp}{{\mathbf{p}}}
\newcommand{\vx}{{\mathbf{x}}}
\newcommand{\vy}{{\mathbf{y}}}
\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\hx}{\hat{\mathbf{x}}}
\newcommand{\hy}{\hat{\mathbf{y}}}

% Unit vectors - bold with hats
\newcommand{\hvx}{\mathbf{\hat{x}}}
\newcommand{\hvy}{\mathbf{\hat{y}}}
\newcommand{\hvm}{\boldsymbol{\hat{\mu}}}
\newcommand{\hvn}{\mathbf{\hat{n}}}
\newcommand{\bchi}{\hat{\bb{\chi}}}

% Other math shortcuts
\newcommand{\vphi}{{\varphi}}
\newcommand{\ham}{\hat{H}}
\newcommand{\tphi}{\tilde{\phi}}
\newcommand{\bpsi}{\bar{\psi}}
\newcommand{\bz}{\bar{z}}
\newcommand{\tr}{\text{tr}}
\newcommand{\sd}[1]{\slashed{#1}}

% Math commands - General
\newcommand{\final}{\comment} %comment out figures that take a long time to load
\renewcommand{\o}{\over}
\newcommand{\eq}[1]{\begin{align}#1\end{align}}
\newcommand{\eql}[1]{\begin{align}#1\end{align}}

% Brackets
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}
\newcommand{\abs}[1]{\left| #1 \right|}

% Spacing and newlines in math mode
\newcommand{\nt}{\notag\\}
\newcommand{\tnl}{\\[1.5ex]}

% Math typesetting commands
\let\spt\mathcal
%\renewcommand{\v}{\boldsymbol}%
\let\v\mathbf
\newcommand{\ti}{\tilde}
\newcommand{\bb}{\boldsymbol}
\newcommand{\ph}{\phantom}

%Greek letters
\newcommand{\ep}{\epsilon}
\newcommand{\vep}{\varepsilon}
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\renewcommand{\d}{\delta}
\newcommand{\g}{\gamma}
\newcommand{\n}{\nu}
\newcommand{\m}{\mu}
\renewcommand{\t}{\tau}
\newcommand{\s}{\sigma}
\newcommand{\w}{\omega}
\renewcommand{\th}{\theta}
\newcommand{\vth}{\vartheta}
\newcommand{\vph}{\varphi}
\newcommand{\lam}{\lambda}
\renewcommand{\r}{\rho}
\newcommand{\Lam}{\Lambda}
\renewcommand{\k}{\kappa}

% Math Symbols
\let\ptl\partial
\renewcommand{\dag}{\dagger}
\newcommand{\ninfty}{{-\infty}}
\newcommand{\fr}{\mathcal{F}}
\newcommand{\id}{\mathds{1}}
\newcommand{\Zt}{\mathds{Z}_2}
\newcommand{\Z}{\mathds{Z}}
\renewcommand\Re{\operatorname{\mathfrak{Re}}}
\renewcommand\Im{\operatorname{\mathfrak{Im}}}
\def\dbar{{\mathchar'26\mkern-12mu d}} %d-slash using in thermodynamics

% Arrows
\newcommand{\ua}{\uparrow}
\newcommand{\da}{\downarrow}
%\renewcommand{\ra}{\rightarrow}
\newcommand{\la}{\leftarrow}

% Hyperbolic trig functions
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\csch}{csch}
\DeclareMathOperator{\arcsinh}{arcsinh}

% Jacobi theta functions
\newcommand{\jthetac}[2]{\vartheta\begin{bmatrix}#1\\#2\end{bmatrix}}
\newcommand{\jThetac}[2]{\Theta\begin{bmatrix}#1\\#2\end{bmatrix}}

%Raise box for Feynman diagram
\newcommand{\mf}[1]{\raisebox{-0.4\height}{\hbox{ {#1}}}}
\newcommand{\mff}[1]{\raisebox{-0.48\height}{\hbox{ {#1}}}}

%Allow margin change for part of page
\def\changemargin#1#2{\list{}{\rightmargin#2\leftmargin#1}\item[]}
\let\endchangemargin=\endlist 

% Itemize shortcut
\newcommand{\lst}[1]{\begin{itemize}#1\end{itemize}}
\newcommand{\pt}{\item}

%table of contents
\usepackage{tocloft} 
% \cftpagenumbersoff{chapters}
\addtocontents{toc}{\cftpagenumbersoff{chapter}}
\addtocontents{toc}{\cftpagenumbersoff{section}}

\setlist[enumerate]{leftmargin=*}

%fancy overbar
%\newsavebox\myboxA
%\newsavebox\myboxB
%\newlength\mylenA
%
%\newcommand*\xoverline[2][0.75]{%
%    \sbox{\myboxA}{$\m@th#2$}%
%    \setbox\myboxB\null% Phantom box
%    \ht\myboxB=\ht\myboxA%
%    \dp\myboxB=\dp\myboxA%
%    \wd\myboxB=#1\wd\myboxA% Scale phantom
%    \sbox\myboxB{$\m@th\overline{\copy\myboxB}$}%  Overlined phantom
%    \setlength\mylenA{\the\wd\myboxA}%   calc width diff
%    \addtolength\mylenA{-\the\wd\myboxB}%
%    \ifdim\wd\myboxB<\wd\myboxA%
%       \rlap{\hskip 0.5\mylenA\usebox\myboxB}{\usebox\myboxA}%
%    \else
%        \hskip -0.5\mylenA\rlap{\usebox\myboxA}{\hskip 0.5\mylenA\usebox\myboxB}%
%    \fi}
%    \makeatother

